Fatigue and mental underload further pronounced in L3 conditionally automated driving: Results from an EEG experiment on a test track

Drivers' role changes with increasing automation from the primary driver to a system supervisor. This study investigates how supervising an SAE L2 and L3 automated vehicle (AV) affects drivers' mental workload and sleepiness compared to manual driving. Using an AV prototype on a test track, the oscillatory brain activity of 23 adult participants was recorded during L2, L3, and manual driving. Results showed decreased mental workload and increased sleepiness in L3 drives compared to L2 and manual drives, indicated by self-report scales and changes in the frontal alpha and theta power spectral density. These findings suggest that fatigue and mental underload are significant issues in L3 driving and should be considered when designing future AV interfaces.

==> notes.tex <==
reseacrch questions

How accurate are sleepiness estimates from use of EEG-based drowsiness detection systems?* What other factors affect drivers' propensity for sleepiness?
What factors affect drowsiness when driving?
How much of a role will sleepiness play in highly automated driving?
How much sleepiness is related to highly automated driving?
Will automation make people more or less drowsy?
How can we design a clear and effective user interface for an automated vehicle?
What are the factors that lead people to fall asleep while driving? What safety precautions do existing cars already have to counteract this problem?
What interventions have been developed to combat driver drowsiness and what research is needed to improve them?
What does drowsiness cause to happen inside an automated vehicle (e.g. what behaviors trigger a warning signal)

